OmniFair: A Declarative System for Model-Agnostic Group Fairness in Machine Learning

Machine learning (ML) is increasingly being used to make decisions in our society. ML models, however, can be unfair to certain demographic groups (e.g., African Americans or females) according to various fairness metrics. Existing techniques for producing fair ML models either are limited to the type of fairness constraints they can handle (e.g., preprocessing) or require nontrivial modifications to downstream ML training algorithms (e.g., in-processing). We propose a declarative system OmniFair for supporting group fairness in ML. OmniFair features a declarative interface for users to specify desired group fairness constraints and supports all commonly used group fairness notions, including statistical parity, equalized odds, and predictive parity. OmniFair is also model-agnostic in the sense that it does not require modifications to a chosen ML algorithm. OmniFair also supports enforcing multiple user declared fairness constraints simultaneously while most previous techniques cannot. The algorithms in OmniFair maximize model accuracy while meeting the specified fairness constraints, and their efficiency is optimized based on the theoretically provable monotonicity property regarding the trade-off between accuracy and fairness that is unique to our system. We conduct experiments on commonly used datasets that exhibit bias against minority groups in the fairness literature. We show that OmniFair is more versatile than existing algorithmic fairness approaches in terms of both supported fairness constraints and downstream ML models. OmniFair reduces the accuracy loss by up to $94.8\%$ compared with the second best method. OmniFair also achieves similar running time to preprocessing methods, and is up to $270\times$ faster than in-processing methods.

==> coverletter.tex <==


\begin{center}
    {\LARGE Revision for SIGMOD'21 Paper 31: \\OmniFair: A Declarative System for Model-Agnostic Group Fairness in Machine Learning}

\end{center}

\bigskip
We are very grateful to reviewers for this opportunity to improve upon our manuscript. In this cover letter, we grouped related comments for better organization. In our revised manuscript, we have highlighted \rev{the modifications in blue}. 


\bigskip
{\huge \stitle{Section 1: Response to Meta-Reviews and Related Comments}}


\bigskip
\begin{tcolorbox}

\textbf{M1.} Improve the theoretical statements as described by reviewer 1, and state any assumptions clearly.

\textbf{R1.O1.} Your "Theorem 1" really shouldn't be a theorem. It's just a direct application of the method of lagrange multipliers. Additionally, I think it needs some additional assumptions to be valid. For example, consider the case where $AP(x) = -(x-1)^2$ and $FP(x) = sinh(x)$. Then (13) has no maximum for any nonzero lambda. The error seems to be in assuming that the function has a maximum when it needn't. 

\textbf{R1.O2.} Theorem 2 is similarly weak. This is a standard result in the optimization theory of lagrange multipliers.

\textbf{R1.O3.} Theorems 3 and 4 are weak for reasons analogous to the issues with Theorems 1 and 2.
\end{tcolorbox}

\stitle{Response.} We have revised our theoretical statements as suggested by R1. In particular, we did the following.
\begin{itemize}
    \item We downgraded all theorems to lemmas (\rev{see ~\Cref{theo:feasibility_single}, ~\Cref{thm:monotonicity_single_lamda}, ~\Cref{th:impossibility}, and~\Cref{thm:monotonicity_multiple_lamda}}), as they are indeed inspired heavily from results in Lagrangine multipliers in convex optimization theory.

    \item We have explicitly stated the assumption \rev{in ~\Cref{theo:feasibility_single}} for it to hold theoretically, i.e., the strong duality assumption between ~\Cref{equ:original} and~\Cref{equ:reg2}.
    
    \item We have discussed the assumption \rev{in the text following ~\Cref{theo:feasibility_single}}. Specifically, we pointed that in cases when the strong duality assumption fails to hold, the Lagrangian dual is still commonly used in practice to obtain a good approximate solution to the primal problem. We also referenced our empirical results, which showed that the strong duality assumption indeed has little practical implications --- we used four ML models, three of which have a non-convex loss, (including a new neural network model we added in this revision in response to R3.O5), and OmniFair performs well under all four tested models.
    
    \item We also highlighted a small but important difference between our ~\Cref{thm:monotonicity_single_lamda} and standard results in Lagrangian multipliers \rev{in the text following ~\Cref{thm:monotonicity_single_lamda}}, that is, the direction of monotonicity depends on the sign of the hyperparameter $\lambda$.  
    
    \item We have also updated \rev{the descriptions of ~\Cref{th:impossibility} and~\Cref{thm:monotonicity_multiple_lamda}} similarly.
    
    
\end{itemize}



% R1.O1
% (1) Indeed, Thrm 1 needs an assumption of strong duality between Eq (11) and (13), i.e. , the optimum solution to the primal problem equals to  the optimum solution to the dual. If the primal problem is convex, strong duality holds under mild conditions (c.f. Chap 5.2.3 in Convex Optimization by Boyd). In the counterexample, sinh(x) is not convex, and the strong duality fails to hold. Note that even without the assumption, the lagrangian dual is still used in practice to give a good approximate solution for the primal problem. We will precisely state and discuss the assumption.

% (2) We note that the strong duality assumption has little implication on empirical results. We used three ML models, two of which (RF and XGBoost) have a non-convex loss (i.e., AP). OmniFair performs well under all three models. We will add another non-convex model Neural Network, suggested by R3.

% (3) We will downgrade Thrm 1 to a lemma.

% R1.O2
% (1) For Thrm 2, one difference between our setting and typical results in Lagrangian multipliers is that the direction of the monotonicity property for AP is different between the pos and the neg range of lambda (c.f. Eq (18) and (19)).  

% (2) Nevertheless, we agree that Thrm 2 closely relates to results in Lagrangian multipliers, and we will change it to a lemma.

% R1.O3
% We will revise Thrm 3 and 4 similarly.





\bigskip
\begin{tcolorbox}

\textbf{M2.} Position the work and motivation properly to avoid overstatements and overclaiming, and clarify the scope and applicability of OmniFair.

\textbf{R2.O1} Overstatements on Constraints and Guarantees: The motivation and goals are very compelling, but unfortunately the technical content did not actually solve the given problem, at least not in the sense of a constraint or even soft constraint (in expectation <= eps). The proposed approach is still very useful, but I would recommend to tear down unnecessary overstatements and make the guarantees and restrictions clear upfront. This should include any guarantees you can make on satisfying the constraints (on train, validation, test data), where and how this is evaluated (train/validation set, which both bear the danger of leaking information given many runs with different lambdas), and the statements on monotonicity. Again, you might be able to show monotonicity for the training data, but not for the test data. For example, Bill Howe's DEEM'20 keynote gave an example (video, 43:43) where stricter fairness constraints led to higher accuracy on the test set due to better generalization (similar to regularization terms). I would recommend to be very careful and specific when trying to position this as a theorem. In order to make room for the additional discussion, I would recommend to cut the "proof" of theorem 2, cut Example 2 (which is not sufficiently explained anyway), and cut the end of Example 5.
\end{tcolorbox}

\stitle{Response.}  We have carefully revisited claims made in the paper, and have made the following modifications throughout the paper. 

\begin{itemize}
    \item In regular ML regime without fairness considerations, for a given ML algorithm ${\mathcal{A}}$, one trains an ML model on a training set using ${\mathcal{A}}$, and whether the model generalizes to the unseen test sets or not depends largely on the size of the training set. If one wishes to tune certain hyperparameters in ${\mathcal{A}}$, then a separate validation set is usually used to avoid overfitting the hyperparameters to the training set by finding a hyperparameter setting with the maximum validation accuracy. 
    %How good are the hyperparameter settings found depends largely on the size of the validation set. 
    
    %standard ML training algorithms with hyperparameters (without fairness considerations), one seeks to tune hyperparameters such that the trained model with a particular hyperparameter setting has the maximum validation accuracy; of course, such a hyperparameter setting may not necessarily be the choice for a given test set. 
    
    In OmniFair, for a given ML algorithm ${\mathcal{A}}$, we treat $\lambda$ as a hyperparameter that controls accuracy-fairness trade-off. To avoid overfitting $\lambda$ on the training set (as we need to train multiple times using different $\lambda$ values), we similarly use a separate validation set to evaluate the goodness of a $\lambda$ value. In particular, we randomly split $D$ into a $D_{train}$ and a small $D_{val}$. We use $D_{train}$ for training ML models for different $\lambda$ values (i.e., when applying $\mathcal{A}$), and use $D_{val}$ for evaluating ML models (i.e., when calculating $FP(\theta)$ and $AP(\theta)$). Our goal is to pick a value for $\lambda$ such that the model trained with that $\lambda$ value would have the maximum validation accuracy while satisfying the fairness constraint on the validation set. We have clarified the use of validation set \rev{at the end of Section~\ref{sec:tuning_lambda_validation}}. 
    
    \item We further stated  \rev{at the end of Section~\ref{sec:tuning_lambda_validation}} that while the use of a separate validation set when tuning $\lambda$ helps with the generalizability of the trained model, there is still no guarantee that the trained model will satisfy the declared fairness constraints on arbitrary unseen test sets. However, a larger validation set is better at ensuring that the accuracy and fairness numbers obtained on the validation set are close to those evaluated on a unseen test set.
    
    \item We also added an experiment to empirically observe the impact of validation set size on test accuracy and test bias. We first partition the COMPAS dataset into 60\% training, 20\% validation, and 20\% test. We vary the validation set size by using a subset of 20\% validation split, and use the same training and test set. As shown in \rev{Figure~\ref{fig:validation} in Section~\ref{sec:exp}}, where the input fairness constraint is to enforce the SP difference between two groups to be within $\epsilon = 0.03$, we can see that a too small validation set fails to generalize well (the test bias is bigger than 0.03); as we increase the validation set, the test set behavior stabilizes and its bias is close to 0.03.  
    
    %a too small validation set indeed can fail to generalize well, i.e., the bias ; with bigger validation set, the test set behavior stabilizes. 
    %\hantian{We added an experiment with Figure~\ref{fig:validation} in Section~\ref{sec:exp} that showed that as the validation set size grows, we would be able to achieve better test fairness, which means the fairness constraint generalizes better to the test set.}\xu{We added an experiment that showed that....} 
    
    \item We have also made the above restrictions more upfront by adding a discussion paragraph \rev{immediately following the formal problem definition in Section~\ref{sec:declarative}} as well as a clarification paragraph \rev{in the key features part of Section~\ref{sec:intro}}.
    
    %Hence, OmniFair has the same limitation in terms of generalization as regular ML training algorithms with hyperparameters.
    
    \item We have modified \rev{Lemma~\ref{thm:monotonicity_single_lamda}} as well as \rev{Lemma~\ref{thm:monotonicity_multiple_lamda}} to state explicitly that the monotonicity property (and the marginal monotonicity property) is only theoretically valid on the training set.  We also clarified \rev{at the end of Section~\ref{sec:monotonicity_single}} why the monotonicity property, which is only theoretically true on the training set, is nevertheless practically useful for designing efficient methods of tuning $\lambda$ using the validation set. 
    %Nevertheless, it provides a practically efficient way to search over all possible $\lambda$ values to find the one with the maximum validation accuracy while satisfy the fairness constraint using the validation set. 
    This is based on the assumption that the training, the validation set, and the unseen test set are from the same distribution, and hence a model with a higher or lower $AP(\theta)$ or $FP(\theta)$ on the training set would also most likely have a higher or lower $AP(\theta)$ or $FP(\theta)$ on the validation set or the unseen test set.
    
    %for two models $\theta_1$ and $\theta_2$ trained using $\lambda_1$ and $\lambda_2$, respectively 
    %In OmniFair, instead of using random search or grid search for tuning $\lambda$, we leveraged the monotonicity property. Of course, the monotonicty property theoretically is only true on the training set. Nevertheless, it provides a practically efficient way to search over all possible $\lambda$ values to find the one with the maximum accuracy while satisfy the fairness constraint using the validation set. 
%    \item We treat lambda similarly to ML model hyperparameters. We use the training set to train a model for a given lambda, and we use a separate val set to select the best lambda that satisfies the constraint, which helps generalization to the unseen test. We agree that there is still no guarantee on the test set.
    %\item  We will state our guarantees and generalizations more precisely throughout. We will also add an empirical study by varying the val set size and observe its impact on test for both fairness and accuracy.
    
    
    \item A prior work FairPrep~\cite{schelter2019fairprep} showed that many existing algorithmic fairness work only focused on tuning the hyperparameter that controls the accuracy-fairness trade-off, and neglected to tune the traditional ML algorithm hyperparameters, which can strongly impact the reported results. Thus, we clarified further \rev{in the hyperparameter tuning paragraph in Section~\ref{sec:exp}} our procedure for evaluating different methods. Specifically, we randomly split each dataset to 60\% training, 20\% validation, and 20\% test. All hyperparameters (including both traditional ML hyperparameters that are specific to an ML algorithm and hyperparameters that are specific to fairness enforcement algorithms) are tuned using the validation set, and all reported results are on the unseen test set. All results reported are the average performance of 10 different random splits.
    
    \item We have also clarified the scope and applicability of OmniFair in terms of the supported fairness constraints \rev{at the end of Section~\ref{sec:3:custom}}. Please see our response to \textbf{M3} below for more details on this.
    
    \item We take all the suggested methods to make room for new contents, including cutting proof of Lemma~\ref{thm:monotonicity_single_lamda}, cutting the original Example 2, and cutting the end of Example~\ref{ex:cutomized_metric} (original Example 5). 
\end{itemize}



\bigskip
\begin{tcolorbox}

\textbf{M3.} Clarify the writing with respect to fairness constraints and specifications.


\textbf{R2.O2} Fairness Specification: The overview of group fairness constraints is a great starting points. Then, Definition 1 (fairness constraints over pairs of groups) also makes sense. However, the definition in Section 5, especially $FP(\theta)$ is inconsistent to this previous definition as it defines $FP(\theta) = f(h_{\theta}, g_1) - f(h_{\theta}, g_2)$ - so suddenly the constraints f are only defined over individual groups. Furthermore, why is a single grouping function sufficient for supporting multiple constraints that might require different grouping functions. As the fairness specification and abstraction, might be reused by other works, it would be good to clean this up. 

\textbf{R2.O2 (updates after rebuttal.)} Thanks for the clarifications, I indeed overlooked the differentiation into specification and constraint, and I appreciate the intend to consolidate this description.


\textbf{R2.O3} Unsupported Fairness Constraints: Group constraints is a very general term. I would recommend to be more specific which kinds of constraints OmniFair supports, including the types of custom constraints. If unspecified, readers associate a strong meaning with custom constraints in terms arbitrary UDFs. Examples that may be hard to express are (1) disjunctions of attributes (the paper talks about conjunctions, but disjunctions would mean that the same tuple may appear in multiple groups), (2) regression problems with monotonicity constraints (e.g., as a certain feature - of some groups - increases, the target variable needs to monotonically increase), and (3) constraints among groups of groups (not just pairs). Furthermore, please add the intuition how the weights are derived for arbitrary custom constraints, while working for all algorithms including algorithms like SVMs with non-linear kernels.

\textbf{R2.O3 (updated comments after rebuttal)}  I did not understand the statement "OmniFair supports non-disjoint groups" in the rebuttal. Did you want to say "supports only disjoint groups" (which is fine if the paper gets positioned accordingly), or do you actually support non-disjoint (i.e., overlapping) groups?

\end{tcolorbox}

\stitle{Response.} We have clarified our writing with respect to fairness constraints and fairness specifications as suggested. Specifically, we included the following changes.

\begin{itemize}
    \item We have added \rev{a paragraph following Definition~\ref{def:fairness}} to highlight the difference between a fairness constraint and a fairness specification. Specifically, we noted that  Definition~\ref{def:fairness} defines two concepts: fairness specification and fairness constraint. A specification is a triplet $(\at{g}, \at{f}, \varepsilon)$ that users specify. A given specification can induce multiple constraints, one for each pair of groups given by $\at{g}$. To specify multiple constraints that require different grouping, users need to provide multiple specifications. Section~\ref{sec:single} handles a single specification that gives one constraint only, i.e., the grouping function generates only two groups. Section~\ref{sec:mutiple} handles multiple constraints, which may be induced by a single specification that generates multiple groups or multiple specifications.
    
    \item \rev{At the end of Section~\ref{sec:3:custom}}, we have added a paragraph to summarize the scope and limitations of OmniFair. Specifically, OmniFair currently supports group fairness constraints defined in the context of supervised binary classification problems. In terms of the grouping function, users can write any logic for forming groups as long as the function returns more than two groups of tuples, and any pair of groups \textbf{does not necessarily need to be disjoint} (see the last bullet point for example weight calculation in such cases). In terms of the fairness metric function, OmniFair can only support those metrics that can be expressed as a linear combination of the identify function (c.f. Definition~\ref{sec:declarative:function}). We further note that OmniFair can only constrain the difference of a given metric between a pair of groups to be within a threshold, i.e., $|\at{f}(h,g_i) - \at{f}(h,g_j)| \leq \varepsilon$. For example, we do not support the constraining of the division of a given metric between two groups to be within a threshold, and we do not support constraints expressed over more than pairs of groups.

    
    
    \item  \rev{At the beginning of Section~\ref{sec:black_box_given_lambda}}, we added some intuition of how example weights are derived for any constraints $FP(\theta)$ permitted by OmniFair. Specifically, we stated that the key to solving~\Cref{equ:reg2} (i.e., $ \max_{\theta} AP(\theta) + \lambda FP(\theta)$) for any constraints $FP(\theta)$ is to transform it into a weighted regular ML optimization problem, which would then allow us to use any ML algorithms. Intuitively, this is possible because both $AP(\theta)$ and those $FP(\theta)$ permitted by OmniFair are expressed as linear combinations of $\mathbbm{1} (h_{\theta}(x_i)=y_i)$, and hence the overall $AP(\theta) + \lambda FP(\theta)$ can be converted into a weighted regular ML optimization problem.
    
    \item We further clarified \rev{in the body of Section~\ref{sec:black_box_given_lambda}} about the exact calculation of example weights for arbitrary $FP(\theta) = \sum_{i \in g_1} (c_i^{g_1} \mathbbm{1}_i + c_0^{g_1}) -  \sum_{i \in g_2} (c_i^{g_2}\mathbbm{1}_i + c_0^{g_2})$, where $c_i^{g_1}, c_0^{g_1}, c_i^{g_2}, c_0^{g_2}$ are provided by users when they define the fairness metric function (c.f. Definition~\ref{sec:declarative:function}). For the points in $D$ that belong to $g_1$ only, their weights are $w_i = 1 + N \lambda c_i^{g_1}$; and for data points in $g_2$ only, their weights are $w_i = 1 - N \lambda c_i^{g_2}$. For the points that belong to both $g_1$ and $g_2$ (\textbf{as two groups may be overlapping}), their weights are $w_i = 1 + N \lambda c_i^{g_1} - N \lambda c_i^{g_2}$. For points that belong to neither group, their weights are $w_i = 1$.
\end{itemize}





\bigskip
\begin{tcolorbox}

\textbf{M4.} The authors should further clarify the distinction and contributions of OmniFair with respect to prior work. The reviewers remain concerned about the similarity with prior techniques and need to be convinced of the significance of the contributions.


\textbf{R3.O1} The core techniques (Lagrangian method and reduction) are very similar to those made in prior work (reference[4]), however the distinction is not clear enough to understand the paper's novel technical contributions.

\end{tcolorbox}

\stitle{Response.}   OmniFair is different from [4] in the following three major aspects, which we have summarized and clarified at \rev{the end of  Section~\ref{sec:related_work}}.
\begin{itemize}
    \item \textbf{Larger Scope of Supported Constraints.} OmniFair supports a wider ranger of constraints. While both OmniFair and [4] support statistical parity and equalized odds, OmniFair additionally support predictive parity (i.e., FOR and FDR) compared with [4]. It is explicitly stated in [4] (at the end of Page 2 in [4]) that it does not support fairness constraints whose conditional moments depend on $h_{\theta}$ (such as FOR and FDR). This means that \textbf{[4] does not support any constraints whose associated example weights are parameterized by $h_{\theta}$} using OmniFair's terminology. 
    \item \textbf{More User-friendly Constraint Specification.} For those constraints that both OmniFair and [4] can support,  OmniFair is significantly more user-friendly in terms of constraint specification due to our declarative interface, \textbf{a fundamental database idea and a key contribution of the paper}. In OmniFair, users simply need to provide the grouping function, the fairness metric function, and the threshold, OmniFair will automatically construct the implied constraints and solve the constrained optimization problem, which is an entirely transparent process to users. In contrast, users of [4] would have to hard-code the desired constraints in terms of linear inequalities on conditional moments (Equation (1) in [4]). Indeed, when we examined the codebase of [4] (\url{https://github.com/fairlearn/fairlearn}), the two constraint types (demographic parity and equalized odds) that [4] uses as examples in the paper are hard coded into the codebase. If users would like to use [4] for those constraints that it can support theoretically (e.g., Example~\ref{ex:cutomized_metric} in this paper), they need to change their codebase by defining a new constraint class and implementing two methods: \textit{events} and \textit{utilities}, which is a highly non-trivial task if users are not familiar with the codebase. 
    %Among those two methods, \textit{events} are described in the paper, whereas \textit{utilities} is not even mentioned in the paper.
    
    %which makes it even harder to implement. 
    
    %modify the constraints as well as the optimization procedure accordingly. \xu{: this part needs to be refined. how they are hard-coded?} \hantian{Each of the constraint is defined as a constraint class that is passed to the classifier. So theoretically for a new constraint, you need to write the constraint as a new constraint class according to its definition(e.g. how to calculate this metic), and there is no need to change the optimization procedure.}
    \item \textbf{Faster Optimization Procedure.} For those constraints that both OmniFair and [4] can support, as rightfully pointed out by R3.O1, both approaches translate the constrained optimization problem into an unconstrained optimization problem using a similar idea of Lagrangian multipliers. However, OmniFair and [4] solve the unconstrained optimization problem differently, and OmniFair is \textbf{about 10 times faster on average}, \rev{which we highlight in Sec~\ref{sec:exp}}. In particular, OmniFair leverages the monotonicity property for designing an efficient hyperparameter tuning procedure, which invokes the training algorithm $\mathcal{A}$ as few times as possible (see complexity analysis in Sec 5).  In [4], the unconstrained optimization problem is further transformed into a saddle point finding problem, which is known to be difficult to solve. Indeed, [4]  states that the number of iterations (i.e., invocations to  $\mathcal{A}$) needed is $O(1/v^2)$, where $v$ is a suboptimality hyperparameter, which is set to around 0.001 in their codebase. 
    %%    
    Empirically, we observe that [4] needs much fewer iterations than their theoretical bound, which is similar to the number of iterations required by OmniFair across different datasets. The reason for why OmniFair is much faster than [4] is because [4] is much slower in completing one iteration than OmniFair. In OmniFair, the main cost of each iteration is to invoke the ML algorithm $\mathcal{A}$, and there is no extra computation. In contrast, each iteration of [4] needs to invoke $\mathcal{A}$ multiple times (one time to calculate $h_t$ and eight times to calculate \underline{$L$} in their implementation). In addition, when we examined their codebase, we found that within each iteration,  it also needs to run a linear programming for saddle point optimization over the convex hull of already trained classifiers to find the best $\lambda$ of current iteration, which is not described in their Algorithm 1 of [4]. The performance gap of OmniFair and [4] is reported in Figure~\ref{fig:exp_efficiency_sp}. 
    
    %The extra computation and multiple invocations of $\mathcal{A}$ are the reasons making [4] m
    
    %However, for each iteration,  [4] needs to invoke the classifier multiple times in their implementation of Algorithm 1 in their paper: once to calculate $h_t$, eight times to calculate \underline{$L$}, and it also needs to run a linear programming for saddle point optimization over the convex hull of already trained classifiers to find the best $\lambda$ of current iteration, which is not described in their Algorithm 1. All those computation make each iteration of [4] runs slowly, while OmniFair only need to invoke the classifier once each iteration, which is the main reason for why OmniFair runs much faster than [4] as reported in Figure~\ref{fig:exp_efficiency_sp}. 
    
    %Empirically, we observe that OmniFair needs 15 invocations of $\mathcal{A}$ on average, while [4] needs 6 invocations, \hantian{However, each invocation of OmniFair only needs to retrain the model once, on Compas dataset. For [4], each invocation needs to train the model multiple times for the saddle-point optimization.}, which is the main reason for why OmniFair runs much faster than [4] as reported in Figure~\ref{fig:exp_efficiency_sp}. \xu{Fill in those XXX.}
\end{itemize}


\bigskip
\begin{tcolorbox}


\textbf{M5.} With respect to prior work, the following paper was brought up in the discussion: 

\smallskip
Philip S. Thomas, Bruno Castro da Silva, Andrew G. Barto, Stephen Giguere, Yuriy Brun, and Emma Brunskill, Preventing Undesirable Behavior of Intelligent Machines, Science, vol. 366, no. 6468, 22 November 2019, pp. 999–1004.

\smallskip
The current submission states that existing work does not support multiple constraints in a practical way, which seems to be contradicted by this publication, which describes an in-processing method that supports multiple constraints. The reviewers believe it is highly relevant, especially when discussing user contracts and fairness specifications. The authors are asked to look into the work cited above, discuss any distinctions, and contrast it with OmniFair.


\end{tcolorbox}

%We compared with the above paper. Thomas et. al.[2] present a nice framework such that it could guarantee fairness on test data. They also allow users to specify undesired behavior to avoid and use what they called Seldonian or Quasi-Seldonian optimization to optimize for the objective function. We extended the discussion in section 2 to show the comparisons. 

\stitle{Response.} We thank the reviewers for pointing out the 2019 Science paper~\cite{thomas2019preventing}, which we were not aware of. We have carefully studied the main paper, the 73-page appendix that described its approaches in much more detail, as well as its codebase (\url{https://zenodo.org/record/3490615#.X5bosYhKguU}). We detail our comparisons with~\cite{thomas2019preventing} in the following.
%which are summarized and added to \rev{Section~\ref{sec:related_work}} in the revised paper. 




\begin{itemize}

    \item \textbf{High-level differences between OmniFair and ~\cite{thomas2019preventing}.}  OmniFair and~\cite{thomas2019preventing} share the same overall objective, that is, making it dramatically easier for users of ML algorithms to specify and regulate bias or undesirable behavior without having to think about how to modify ML training algorithms. However, they take fundamentally different approaches for doing so. 
    
    %They share two fundamentally different approaches for doing so. 
    
    \begin{itemize}
        \item  OmniFair proposes a concrete declarative interface for defining fairness constraints, which can be enforced with \textbf{any existing black-box ML algorithms} without modifying them. In this way, users need not think about modifying ML algorithms, and focus on specifying fairness constraints.
        
        \item In contrast, ~\cite{thomas2019preventing} mainly proposes a principled framework for \textbf{ML researchers or engineers} for designing \textbf{new ML algorithms} that can support fairness constraints. Once a new ML algorithm is designed, end users can use it directly together with constraints it supports without worrying about the internals of the new ML algorithm. 
        %%%
        The framework proposed in ~\cite{thomas2019preventing} for designing new ML algorithms with fairness interfaces consists of three steps: (i) defining the objective function of the new ML algorithm; (ii) defining the interface that the users will use to specify fairness constraints; and (iii) creating the training algorithm to solve the objective function defined in (i) subject to any constraints defined via the interface defined in (ii). It is not surprising, and also stated explicitly in~\cite{thomas2019preventing}, that  the primary difficulty of instantiating the framework (which has to involve ML researchers or engineers) is to specify the class of allowed fairness constraints  that are compatible with the ML training algorithm to be created. 
    \end{itemize}
    \smallskip
    
    As we can see, users of OmniFair have the freedom to pick any existing ML algorithms, while users of ~\cite{thomas2019preventing} are tied with a particular new ML algorithm (to be designed by ML researchers) if they would like to specify fairness constraints using the associated interface (to be designed by ML researchers). We have now discussed ~\cite{thomas2019preventing} in \rev{related work in Section~\ref{sec:related_work}}.
    
    
   
    % In contrast, 
    
    % However, the primary contributions of OmniFair and~\cite{thomas2019preventing} are vastly different. OmniFair proposes a concrete system with a defined interface for users to specify fairness constraints that can be used in conjunction with any ML algorithms. On the other hand, as stated in~\cite{thomas2019preventing} itself, the primary contribution of~\cite{thomas2019preventing} is the proposal of a framework for designing such ML algorithms and interfaces to achieve the said objective, rather than concrete algorithms or systems that implement the framework (though the paper does provide example concrete algorithms that instantiate the framework, which we will discuss later). 
    
    \item \textbf{Empirical Comparison between OmniFair and a new ML algorithm (CMA-ES) proposed in ~\cite{thomas2019preventing}.} To demonstrate how the framework can be used, ~\cite{thomas2019preventing} includes a concrete new ML algorithm as an instantiation of the framework for supervised classification tasks. We carefully examined the description and the code of that instantiation. We learned that it uses the misclassification rate as the objective function, and it supports  statistical parity, equalized odds, and misclassification rate. It  uses a specific training procedure, called Covariance Matrix Adaptation Evolutionary Strategies (CMA-ES). 
    
    The empirical comparison with CMA-ES is shown as  \rev{in Table~\ref{table:accuracy} in Section~\ref{sec:exp}}. We can see that the customized CMA-ES algorithm can indeed achieve competitive performances; however, since OmniFair works with any ML algorithm, OmniFair can produce a more accurate model by trying different ML algorithms (e.g., OmniFair with XGB on COMPAS is better than ~\cite{thomas2019preventing} with CMA-ES on COMPAS, and OmniFair with NN on LSAC is better than ~\cite{thomas2019preventing} with CMA-ES on LSAC). In addition, OmniFair is more versatile in supported constraints than CMA-ES. 
    
    %We can see that, since OmniFair is free to work with any black-box ML model, there always exists a
    
    %We can see that OmniFair and ~\cite{thomas2019preventing} have similar performances when the end model is the linear model LR across four datasets. However, OmniFair works with any ML algorithm, and hence can produce a more accurate model by trying different ML algorithms (e.g., OmniFair with XGB on COMPAS is better than ~\cite{thomas2019preventing} with LR on COMPAS).
    
    %The framework proposed in ~\cite{thomas2019preventing} for designing ML algorithms with fairness interfaces consists of three steps: (i) defining the objective function of the ML algorithm; (ii) defining the interface that the users will use to specify fairness constraints; and (iii) creating the training algorithm to solve the objective function defined in (i) subject to any constraints defined via the interface defined in (ii). It is not surprising, and also stated explicitly in~\cite{thomas2019preventing}, that  the primary difficulty of instantiating the framework (which is the job of designers of ML algorithms or researchers) is to specify the class of allowed fairness constraints  that are compatible with the ML training algorithm to be created. \smallskip
        
        
        
    %     \begin{itemize}
    %         \item ~\cite{thomas2019preventing} includes a concrete instantiation of the framework for supervised classification tasks. That instantiation only supports linear ML models and works for \hantian{SP, EO and MR}\xu{what types of constraints it support.} This is because it relies on a specific training algorithm \hantian{Covariance Matrix Adaptation Evolutionary Strategies(CMA-ES). CMA-ES is a evolutionary algorithm that could optimize for non-convex objectives. Since neither Seldonian or Quasi-seldonian optimization is convex, CMA-ES is used for optimization. On top of that, both of Seldonian and Quasi-seldonian optimization can only work for linear objective functions.}\xu{XXX what is it} that solves the constrained optimization that can only work for linear objective functions. 
            
    %         \smallskip
            
            
    %         \item OmniFair can be seen as a particular instantiation of the framework with a clearly defined interface for constraint specification as well as a model-agnostic approach for enforcing those constraints for any ML black-box ML models. 
    %     \end{itemize}
    
    % In this sense, OmniFair is much more generic in terms of supported ML models, than the concrete instantiation in ~\cite{thomas2019preventing}. We have also added a comparison with ~\cite{thomas2019preventing} in \rev{Table~\ref{table:accuracy} in Section~\ref{sec:exp}}, \hantian{it showed that OmniFair have comparable accuracy with this science paper on all datasets, and OmniFair supports more classifiers.}\xu{What is it.}
    
    

    
    
    
   
   % However, the objective function they proposed is extremely hard to optimize and only works for linear models for now. For more complicated models, they left the optimization part to the users. In contrast, OmniFair could support any models, because OmniFair doesn’t change the objective function, but does reweighting on the data. In this sense, OmniFair could be seen as an extension to their framework with more classifiers. 
    
    \item \textbf{Constraint satisfaction guarantees on unseen test set.} One benefit of~\cite{thomas2019preventing} is that it provides probabilistic guarantees of fairness constraint satisfaction on unseen test data (hence the name ``Seldonian'', or ``Semi-Seldonian'', depending on whether additional assumptions are made about data distributions). This is essentially achieved by verifying a given model on a separate validation set (depicted as $D_2$ in Figure 1 in ~\cite{thomas2019preventing}), and the guarantees are derived using  concentration bounds, such as Hoeffding's inequality. The tightness of the bounds depends on the size of $D_2$. As stated in our response to \textbf{M2} and \textbf{R2.O1}, OmniFair similarly uses a validation set to verify the satisfiability of declared fairness constraints, however we currently do not provide any formal probabilistic guarantees in terms of constraint satisfaction on unseen test data, which we leave to future work as \rev{mentioned in Section~\ref{sec:conclusion}}.
    
    %One advantage of their model is that it could provide a probabilistic guarantee on test data, while OmniFair couldn’t, as review 2 pointed out. 
    

\end{itemize}
% (1) In Sec 2, we described the technical difference between OmniFair and [4] in terms of weighting on a high level. 

% (2) For constraints that both [4] and OmniFair support, OmniFair shows better results (e.g., Table 4 for SP and Fig 8 for constraints involving multiple groups). This is because OmniFair tunes the weights (via lambda) in a principled way using the monotonicity property, while weight tuning in [4] is heuristics. 

% (3) OmniFair supports predictive parity and customized constraints (due to its novel declarative interface), while [4] does not. 

% (4) We will highlight the difference between OmniFair and [4] clearly in Sec 1, provide more details on the difference between the weighting mechanisms in Sec 2, and compare with [4] directly in Sec 7. 



\bigskip
\begin{tcolorbox}

\textbf{M6.} The reviewers are concerned about the runtime cost of the approach and would like to see a discussion about scaling to large real-world datasets.

\textbf{R3.O2} The approach is very costly (its runtime is two to three orders of magnitude higher than the runtime for some single constraint interventions). The authors should discuss whether their approach can scale to large-real world datasets with millions of records. This might also be an interesting route for future work.
\end{tcolorbox}

\stitle{Response.} During revision, we have added the following discussions regarding the runtime cost of OmniFair. 
%We have added discussions regarding the running time cost of OmniFair in the following three aspects. 

\begin{itemize}
    \item \textbf{Comparison with existing methods.} We agree that OmniFair can have scalability challenges when dealing with large datasets, as OmniFair needs to invoke $\mathcal{A}$ multiple times. However, enforcing fairness constraints comes at a cost, and  in comparison with existing fairness approaches, OmniFair is already superior.  
    
    %While OmniFair is indeed up to slower compared with training without any fairness constraints, as we need to invoke the training algorithm $\mathcal{A}$ many times, it is superior to existing algorithmic fairness approaches
        \begin{itemize}
            \item Compared with existing pre-processing methods, OmniFair achieves comparable running time (c.f. Figure~\ref{fig:exp_efficiency_sp}). However, OmniFair supports a much wider set of constraints, while pre-processing methods only support SP.
            \item Compared with existing in-processing methods, OmniFair is not only faster (from 1.05X to 270X as shown in Figure~\ref{fig:exp_efficiency_sp}), but also achieves better accuracy-fairness trade-off (c.f. Figure~\ref{fig:single_fairness_adult}). 
        \end{itemize}
    We have clarified the above discussions in the \rev{efficiency experiment paragraph in Section~\ref{sec:exp}.}
    
    %(i) OmniFair achieves comparable running time to two preprocessing algos (which only support SP), and is much faster than all in-processing algos (which support more constraints), as shown in Fig 4; (ii) OmniFair is better in terms of accuracy-fairness trade-off compared with all existing algos; and (iii) OmniFair supports customized constraints, while no existing algos can. 


    \item \textbf{An optimization using warm-start.} During revision, we introduced a new warm-start optimization, which is naturally applicable in OmniFair, since OmniFair needs to invoke the ML algorithm  $\mathcal{A}$ multiple times and model parameters trained in the previous iteration can be used as initial parameter values for model training in the next iteration. We conducted an experiment to show the impact of warm-start. As shown \rev{in Table~\ref{table:warmstart} in Section~\ref{sec:exp}}, using warm-start on the LR algorithm leads to an 1.2$\times$ to 3.4$\times$ speed up on different datasets.
    
    %We noticed that we could further speed up OmniFair by using warm-start: a standard technique that we reuse the model weights of last model for initialization. \hantian{We conducted an experiment shown in Table~\ref{table:warmstart} in Section~\ref{sec:exp}, the experiment result shows an 1.3$\times$ to 1.8$\times$ speed up on different datasets.} 
    
    \item \textbf{Future work discussions.} Warm-start does not completely address the scalability problem since some ML algorithms do not permit warm-start (e.g., RF) and running time could still be high for extremely big datasets. As suggested, we have mentioned this challenge as a \rev{future work in Section~\ref{sec:conclusion}}, which could potentially be addressed by parallel model training and  using a smaller sample training set to quickly prune certain $\lambda$ values.
    
    
\end{itemize}



%(3) We used standard datasets in the fairness domain. However, if a dataset has millions of records, OmniFair becomes harder to scale, as one ML run is more costly. One optimization is that a later run could perform a warm start by reusing parameters from a previous run. We will stress-test the scalability of OmniFair, with the warm start idea. 

%1) compare w/ existing method 2) warm start 3) future work: weight a-priori, for models doesn’t support warm start(e.g. Decision tree) do model distillation)


\bigskip
{\huge \stitle{Section 2: Response to other Issues Raised in Reviewer Comments}}
\bigskip


\begin{tcolorbox}

\textbf{R2.O4} Approach Classification: To be honest, I never heard of 'in-processing methods' before. The classification of the introduction made sense, but while going through the paper, I got the impression that OmniFair should actually be classified as pre-processing (or something in between) because OmniFair only modifies tuples weights or replicates the tuples if the algorithms do not support weights. This re-classification would also avoid overstatements like model-agnostic training with custom constraints, which by own admission of the authors is not possible for hard constraints or constraints that cannot be expressed as weights.

\end{tcolorbox}

\stitle{Response.} 

\begin{itemize}
    \item The term in-processing is used in the AIF360 package to classify fairness algorithms, as well as multiple existing work~\cite{friedler2019comparative,barocas2017fairness,pessach2020algorithmic}. 
    
    \item  OmniFair is indeed similar to pre-processing in that it does not modify ML algorithms; however, it is also slightly different because pre-processing algorithms change the data without ever needing to access the ML algorithm $\mathcal{A}$ while OmniFair needs to invoke $\mathcal{A}$  to train multiple models (though via black-box) to decide weights.
    
    \item We choose to classify OmniFair as in-processing since it is most similar to [4] in that both approaches need access to $\mathcal{A}$ but do not need to modify $\mathcal{A}$. Since [4] is referred to as in-processing in the literature (e.g. see Table 2 in~\cite{pessach2020algorithmic}), we similarly classify OmniFair as in-processing. 
    
    \item We appreciate R2 pointing our such subtleties. We have now added a discussion about this \rev{as a comment in Table~\ref{table:baselines}} when we compare different approaches. 
\end{itemize}


%We cl,barocas2017fairnessarifies this and made sure not to overstate OmniFair’s capabilities. \abol{where in the paper did we do this?}

% [R1] S. A. Friedler, C. Scheidegger, S. Venkatasubramanian,
% S. Choudhary, E. P. Hamilton, and D. Roth. A comparative
% study of fairness-enhancing interventions in machine
% learning. In FAT*, 2019.

% [R2] Solon Barocas , Moritz Hardt, Arvind Narayanan. Fairness in Machine
% Learning, Limitations and Opportunities”, 2019 (fairmlbook.org).



\bigskip
\begin{tcolorbox}

\textbf{R2.O5} Hill-Climbing Technique: The introduced hill-climbing technique (independent lambda tuning for all dimensions that to not yet satisfy their constraints) seems a bit ad-hoc, or at least, I do not understand the intuition yet. Wouldn't it be feasible to directly apply old general-purpose optimizers like Nelder–Mead, which does not require a differentiable function but uses a simplex-downhill method. It's slow compared to LBFGS, but very simple and likely faster than the linear search in Algorithm 1 due to expansion and contraction when needed.
\end{tcolorbox}

\stitle{Response.}
\begin{itemize}
    \item We used Hill-Climbing that tunes one dimension while fixing others because we wanted to leverage the marginal monotonicity property. Hill-Climbing produces good results empirically.
    
    \item During revision, we have investigated and tested the suggested Nelder-Mead algorithm. However, at least for now, we failed to find a way to make Nelder-Mead a fit for our problem because it is hard to represent our objective function under the form of Nelder-Mead.  Our objective function is to maximize accuracy, while all fairness constraints are satisfied, while Nelder-Mead's objective function is simply to minimize a loss, i.e., Nelder-Mead does not support constraints. We have experimented with multiple ways to tweak the objective function to incorporate the constraints, including  making the objective function -100 when fairness constraints are not satisfied and 0 when fairness constraints are satisfied and setting the objective function to directly be the degree of violations of the fairness constraints. The returned results are simply not as good as our current Hill-Climbing algorithm. 
\end{itemize}




\bigskip
\begin{tcolorbox}

\textbf{R2.Additional Remarks.} There are a number of minor presentation issues that can be easily fixed:
- Many of plots are very hard to read (very thin fonts, which are barely visible in printed)

- Please, avoid underlining as a form of emphasizing 

- The code in Figure 1 is confusing as its formatted in the color of a comment (but not actually commented). The entire figure is an example, so please just show the code

- The latex macro of OmniFair uses wrong spacing, which leads to unnecessary spaces wherever OmniFair appears directly before punctuation like dots, commas, or parentheses.

- Missing space in "support vector machines(SVM),"

- The text talks about "course-grained" and "find-grained" but it's "coarse-grained" and "fine-grained" 
\end{tcolorbox}

\stitle{Response.} 
We made the plots larger and the fonts thicker, changed all underlines to italic, changed the color of the code in Figure 1 to black instead of green, and fixed the spacing and typos.


\bigskip
\begin{tcolorbox}
\textbf{R3.O3.} It is unfortunate that the proofs reside an extra report and that the paper is not self-contained.
\end{tcolorbox}
\stitle{Response.} Due to the extra discussions and experiments we added in the revision, we are not able to include all proofs in the paper during the revision. However, we now have explicitly stated that our lemmas are  applications of results from lagrangian multipliers in convex optimization~\cite{boyd2004convex}, in response to R1.O1. We hope this will make the paper self-contained, at least for readers who are already familiar with results in lagrangian multipliers. We will make sure that all proofs are contained in the full report~\cite{Full_Report}.

%We recognize that a self-contained paper should include proofs in the main body. However, 

%We note that all reviewers have given comments regarding the theorems. Reviewer 1 (R1.O1) sees our theorems as direct applications of the method of Lagrangian multipliers; Reviewer 2 (R2.O1)  suggests us to cut the proof of Theorem 2 to make room for additional materials; Reviewer 3 (R3.O3) prefers a more self-contained paper with proofs. To take all 




\bigskip
\begin{tcolorbox}
\textbf{R3.O4.} The authors should report additional metrics (not only accuracy) for their experiments such as ROC AUC, assome of the datasets have label skew (e.g., Adult has 76\% negative examples), and bad classifiers can already achieve high accuracy in such cases.
\end{tcolorbox}

\stitle{Response.} We agree that accuracy could be misleading on datasets with severe class imbalance, as a trivial classifier (always predicting to be one class) could already achieve high accuracy. During response, we have reported both ROC AUC and Accuracy as the metric on the skewed dataset (Adult) and plot ROC AUC / Accuracy vs different statistical parity allowance $\varepsilon$ in \rev{Figure~\ref{fig:single_fairness_adult}(a) and (c) in Section~\ref{sec:exp}}.
%Figure~\ref{fig:ROC_AUC} and~\ref{fig:Acc_Adult}. 
We can show that to meet the same $\varepsilon$, for both ROC AUC and accuracy, OmniFair is better than or to to other baseline methods. 
%Due to space limit, we will include this result in the full report~\cite{Full_Report}. 
% \begin{figure}[ht]
% \centering
% \includegraphics[scale=0.5]{figs/ROC_AUC_ADULT.png}
% \caption{\small ROC AUC vs SP on Adult Dataset}
% \label{fig:ROC_AUC}
% \end{figure}

% \begin{figure*}[ht]
% \centering
% \begin{minipage}[t]{0.35\textwidth}
% \centering
% \includegraphics[scale=0.4]{figs/ROC_AUC_ADULT.png}
% \caption*{\small ROC AUC vs SP on Adult Dataset}
% \label{fig:ROC_AUC}
% \end{minipage}
% \centering
% \begin{minipage}[t]{0.35\textwidth}
% \centering
% \includegraphics[scale=0.4]{figs/Accuracy_ADULT.png}
% \caption*{\small Acc vs SP on Adult Dataset}
% \label{fig:Acc_Adult}
% \end{minipage}
%\end{figure*}

\bigskip
\begin{tcolorbox}
\textbf{R3.O5.} 
The experimental section would benefit from experiments on an additional dataset, and the usage of a neural network baseline model as well. 
\end{tcolorbox}

\stitle{Response.} 

\begin{itemize}
    \item We have added a new dataset Bank that predicts if marketing leads to increased product adoption. We have also added Neural Network (NN) as a new ML algorithm. We have updated the \rev{experimental setup in Section~\ref{sec:exp_setup}} to reflect this change.
    \item The result is shown in \rev{Table~\ref{table:accuracy} in Section~\ref{sec:exp}}. We see that for the newly added Bank dataset, in comparison with other fairness approaches, OmniFair performs the best on RF and NN, and is a close second best for the other ML algorithms.  For NN, on Adult, LSAC and Bank dataset, OmniFair is the best performing algorithm, and on the Compas dataset, OmniFair is the second best.
\end{itemize}
%We added another dataset Bank and a Neural Network (NN) baseline. The result is shown in \rev{Table~\ref{table:accuracy} in Section~\ref{sec:exp}}. We see that for the newly added Bank dataset, OmniFair performs best on RF and NN, and the result of other classifiers is a close second best method. For NN, on Adult, LSAC and Bank dataset, OmniFair is the best performing algorithm; on the Compas dataset, OmniFair is also performing reasonablly well (second best).

\bigskip
\begin{tcolorbox}
\textbf{R3.O6.} 
The authors should emphasize the fact that the approach can handle fairness for intersectional groups even stronger.
\end{tcolorbox}

\stitle{Response.} In response to R2.O3,  we have added a paragraph to summarize the scope and limitations of OmniFair in terms of supported constraints \rev{at the end of Section~\ref{sec:3:custom}}. In that paragraph, we have  emphasized how our grouping function can be used to write any logic for forming groups as long as the function returns more than two groups of tuples (e.g., intersectional groups defined over multiple sensitive attributes). We have also mentioned this in \rev{Section~\ref{sec:intro} when we discuss the declarative interface}.

%and any pair of groups do not necessarily need to be disjoint.

%we have added a paragraph to summarize the scope and limitations of OmniFair. Specifically, OmniFair currently supports group fairness constraints defined in the context of supervised binary classification problems. In terms of the grouping function, users can write any logic for forming groups as long as the function returns more than two groups of tuples, and any pair of groups do not necessarily need to be disjoint. In terms of the fairness metric function, OmniFair can only support those metrics that can be expressed as a linear combination of the identify function (c.f. Definition~\ref{sec:declarative:function}). We further note that OmniFair can only constrain the difference of a given metric between a pair of groups to be within a threshold, i.e., $|\at{f}(h,g_i) - \at{f}(h,g_j)| \leq \varepsilon$. For example, we do not support the constraining of the division of a given metric between two groups to be within a threshold, and we do not support constraints expressed over more than a pair of groups or groups of groups.
%Specifically, OmniFair currently supports group fairness constraints defined in the context of supervised binary classification problems. In terms of the grouping function, users can write any logic for forming groups as long as the function returns more than two groups of tuples, and any pair of groups do not necessarily need to be disjoint. In terms of the fairness metric function, OmniFair can only support those metrics that can be expressed as a linear combination of the identify function (c.f. Definition~\ref{sec:declarative:function}). We further note that OmniFair can only constrain the difference of a given metric between a pair of groups to be within a threshold, i.e., $|\at{f}(h,g_i) - \at{f}(h,g_j)| \leq \varepsilon$. For example, we do not support the constraining of the division of a given metric between two groups to be within a threshold, and we do not support constraints expressed over more than a pair of groups or groups of groups.








==> coverletterShepherding.tex <==


\begin{center}
    {\LARGE Revision for SIGMOD'21 Paper 31 Marked as ``Accept With Shepherding'' }

\end{center}

\bigskip
We are very grateful to PC chairs, the meta-reviewer, and the three reviewers for marking this paper as ``Accept With Shepherding'', and for allowing us the opportunity to fix the remaining issues. In particular, \textbf{we have revised the text around lemmas, the lemma statements, and lemma proofs in the appendix, in consultation with our colleagues in optimization theory. We have highlighted the new changes \revnew{in blue}.} 

%reviewers for this opportunity to improve upon our manuscript. In this cover letter, we grouped related comments for better organization. In our revised manuscript, we have highlighted \revnew{the modifications in blue}. 


\bigskip
{\huge \stitle{Section 1: Response to Meta-Reviews and Related Comments}}


\bigskip
\begin{tcolorbox}

\textbf{M1.} The reviewers are generally happy with the revisions, however, they noted that there are still serious issues with the theoretical statements, which require further revisions to correct. While the issues are serious, the reviewers believe they are fixable, and have agreed to accept the paper, conditioned on correcting these problems through shepherding.

\textbf{R1.O1.} There are still some issues, I think, with the revised theory. For example, Lemma 1 still seems to be incorrect; certainly its proof is incorrect. The issue occurs after equation (26) in the supplemental, where you just assume that there is some value $\lambda_F$ for which $\theta_F$ maximizes (26). But no reason is given for why such a $\lambda_F$ must exist! There are also other errors, such as saying "let $\theta_\lambda$ be the value of theta that maximizes the equation" without first showing that such a value exists and is unique.

\textbf{R1.O2.} Lemma 2 has the same issue: no reason is given for why the argmin must exist and/or be unique. Although here, this is a much more minor problem that can be resolved by just assuming the argmin exists.

\textbf{R1.O3} Lemma 3 has the same issue as Lemma 1. No reasoning is given for why the assignment of $\lambda_k$ in the bottom of the proof is not dividing by zero.
\end{tcolorbox}

\stitle{Response.} 
\begin{itemize}
    \item \textbf{[Revision for Lemma 1]} We think that the reason for the confusion regarding our previous Lemma 1 and its proof is because we did not clearly state what is the Lagrangian dual function of the original constrained optimization problem in~\Cref{equ:original}, how the results from Lagrangian dual function are directly applied, and what additional steps we took based on existing results to derive the Lemma. To this end, we made the following changes. 
    
    \begin{itemize}
        \item We have overhauled \revnew{the text before Lemma 1} to provide more context for the statement in Lemma 1. In particular, we first explicitly showed what is the Lagrangian dual function (i.e., ~\Cref{equ:h}) of the original problem in ~\Cref{equ:original} following directly from Chapter 5 in the textbook ~\cite{boyd2004convex}. We then stated the known existing results, again from Chapter 5 in the textbook ~\cite{boyd2004convex}. That is, ~\Cref{equ:h} provides an upper bound to ~\Cref{equ:original} and the bound is tight under the so-called strong duality assumption~\cite{boyd2004convex}. We then showed how we can further simplify ~\Cref{equ:h} into~\Cref{equ:reg2} (which reduces the number of hyperparameters from two to one), and why this simplification is justified. 
        
        \item We have revised  \revnew{the statements in Lemma 1}. In particular, we assume that the primal problem in ~\Cref{equ:original} is feasible. We note that we do not require the optimal solution to ~\Cref{equ:original} to be unique. Hence, in Lemma 1, we now state that let $\theta^*$ be \textbf{an} optimal solution to ~\Cref{equ:original}.  To make Lemma 1 clear, we split Lemma 1 into two parts. The first part is direct applications of Lagrangian dual function, which connects ~\Cref{equ:h} to ~\Cref{equ:original}. The second part formally connects ~\Cref{equ:h} to ~\Cref{equ:reg2}, which is our simplified unconstrained optimization problem with only one hyperparameter.
        
        \item We have revamped \revnew{the proof of Lemma 1 in the appendix of the full paper.} The proof consists of two steps, naturally corresponding to the two parts of Lemma 1. While the first part is directly applying existing results, we nevertheless show the proof of it and discuss the strong duality assumption. We then formally prove the second part of Lemma 1. 
        
        \item We have revised \revnew{the text following the new Lemma 1.} In particular, the revised text discussed the strong duality assumption and how the problem translation is still practically useful even without the strong duality assumption. We then highlighted how Lemma 1 can be used to design algorithms for solving the original problem in~\Cref{equ:original}. That is, given~\Cref{theo:feasibility_single}, we can essentially solve~\Cref{equ:original}  in three steps: (i) enumerating all possible $\lambda$ values; (ii) finding the optimal solution to~\Cref{equ:reg2} for every $\lambda$ value; and (iii) out of all the optimal solutions for different $\lambda$ values, pick the one that has the maximal $AP(\theta)$ while $|FP(\theta))| \leq \varepsilon$. In Sec~\ref{sec:tech:tuning}, instead of enumerating all $\lambda$ values, we design a smart algorithm to search for $\lambda$ efficiently.
        
        %\item We have revised the statement in Lemma 1 to assume that the primal problem ~\Cref{equ:original} is feasible. We also note that we do not require the optimal solution to ~\Cref{equ:original} to be unique. Hence, in Lemma 1, we now state that let $\theta^*$ be \textbf{an} optimal solution to ~\Cref{equ:original}. Our proof works for any optimal solution to ~\Cref{equ:original}. Also, in Lemma 1, we add a statement to show that the Lagrangian dual provides an upper bound to the primal problem, this is true even if the strong duality does not hold and the dual can provide an approximation to the primal problem.
        
        %\item We have revamped our proof for Lemma 1 in the appendix of the full paper. In our original proof, the reason for why such as $\lambda_F$ exist is because of the strong duality assumption. We agree that the original proof is opaque and does not specifically explain how the strong duality assumption is used. 
        
        
        %Our revised  new proof consists of two steps. The first step re-writes ~\Cref{equ:original} without using the absolute term and also gives its Lagrangian dual optimization problem, which is an upper bound to the original problem, then we leverage the strong duality assumption, which means that given an optimal solution $\theta^*$ to the primal problem, we can always find $\lambda_1 > 0$ and $\lambda_2 > 0$ such that the optimal solution is also an optimal solution to the dual problem, which is parameterized by $\lambda_1$ and $\lambda_2$. The Second step shows that we can set $\lambda = \lambda_2 - \lambda_1$, and prove that $\theta^*$ would also be an optimal solution to ~\Cref{equ:reg2}, which completes the proof. We refer reviewers to the appendix for the full proof. 
         
       % \item We added discussions both in text and in the appendix regarding the strong duality assumption. There exists  multiple different conditions for the strong duality assumption to hold (e.g., when the primal problem~\Cref{equ:original} is a linear optimization problem; or when the primal problem is a convex optimization problem and the Slater's condition holds~\cite{boyd2004convex}). Even without the strong duality assumption, the dual problem also called as  Lagrangian relaxation is still commonly used in practice to give a good approximate solution for the primal problem when the primal problem is difficult to solve directly. In \systemx's setting, while we have no way to solve the primal constrained optimization problem in a model-agnostic way, we have developed methods to solve the unconstrained version in a model-agnostic way. In addition, we have empirically shown that for various different ML models where strong duality does not hold (e.g., neural networks, decision tree), \systemx still generates better models than state-of-the-art fairness approaches. 
    \end{itemize}
        
    
%    We have completely changed the proof of Lemma 1 in appendix. The reason for why such $\lambda$ must exist is because our assumption that the strong duality holds. The strong duality means that the optimal value of the primal and dual problem are the same, so there must exists $\lambda$ that optimizes the dual problem, if the primal problem has an optimal value. We stated this in more details in the appendix. In the discussion following Lemma 1, We also specified a case when the strong duality holds is that when both $AP$ and $FP$ are convex, and discussed the case when they are non-convex. If $AP$ or $FP$ is non-convex, then Lemma 1 doesn't hold in most cases, however, we argue that even if strong duality doesn't hold, the Lagrangian dual can usually provide a good approximation to the primal problem because of weak duality.     Also, in the proof, we assume the primal problem is feasible and has an optimal value. It does not need to be unique. 
    
    \medskip
    \item \textbf{[Revision for Lemma 2]} We have \revnew{added assumptions in Lemma 2 to state that we assume the optimal solutions exist} for ~\Cref{equ:lambda_1} and ~\Cref{equ:lambda_2}, as suggested by R1. Again, we do not require the optimal solutions to be unique. Our proof works with any two optimal solutions to ~\Cref{equ:lambda_1} and ~\Cref{equ:lambda_2}, respectively. 
    
    %we assume that the optimal solution exists. One way to ensure that the optimal solution must exist is to make $\theta$ bounded, then according to the Extreme value theorem, there must exist a max and a min.
    
    
    \medskip
    \item \textbf{[Revision for Lemma 3]} After our revision of Lemma 1, Lemma 3 now directly generalizes Lemma 1 and the proof of Lemma 3 follows the proof of Lemma 1. We have similarly revised \revnew{the text before Lemma 3, the statements in Lemma 3, and the proof of Lemma 3 in the appendix}.
    
    % \begin{itemize}
    %     \item We added an assumption in the statement of Lemma 3 to assume that the primal constrained optimization problem is feasible, namely, there exists models that satisfy all given fairness constraints. Again, we do not require the optimal solution to be unique, and we use $\theta^*$ to denote an optimal solution to the primal problem. Similar to Lemma 1, we also added a statement that the dual would be an upper bound to the primal problem, even if the strong duality does not hold.
        
    %     \item We have revamped our proof for Lemma 3 as well. The new proof follows similar steps in the proof of Lemma 1, and avoids the dividing by zero issue. We refer reviewers to the appendix for the full proof. 
    % \end{itemize}
    

    
    %The dividing by zero problem pointed by R1 is true for our original proof for Lemma 3. We note that Lemma 3 is a direct extension of Lemma 1 by changing one constraint to multiple constraints, but the proving steps are the same. So we instead extend the proof for Lemma 1 to prove Lemma 3. We provide more detials in the appendix.
    
\end{itemize}

\bigskip
{\huge \stitle{Section 2: Response to other Issues Raised in Reviewer Comments}}
\bigskip


\begin{tcolorbox}

\textbf{R2.O1}  
\begin{itemize}
    \item The code in Figure 1 uses invalid symbols (e.g., x where you probably mean *)
    \item Figures 2, 3, 4, 5, 9 still have the mentioned font issue (maybe pick a different font closer the paper text)
    \item Missing articles (e.g., "OmniFair achieves [the] smallest accuracy drop in")
    \item Don't use references as nouns (e.g., "used by [48]" - they are meta data)
\end{itemize}

\end{tcolorbox}

\stitle{Response.} 
We updated the corresponding part and fixed the mentioned issues.

==> weighted.tex <==
% !TEX root = main.tex
\section{Single Fairness Metric on Two Groups} \label{sec:single}

\xu{Things we need to convey in this section: }
\begin{itemize}
    \item we focus on one fairness constraint on two groups in this section. The naive constraint optimization problem obviously is hard to solve, and is model-specific. We propose a model-agnostic way of solving the constrained optimization problem. What we have is an ML algorithm ${\cal A}$ that optimizes the empirical loss (explcit or implicit). We will show how to translate the contrained optimization problem into optimizing a weighted empirical loss, which can be solved directly without modifying ${\cal A}$. 
    
    
    \item we can treat a fairness constraint into as a regularization term. How? We need to explain these things: (1) use the loss function as a proxy for the constraint, i..e, $|L(G1) - L(G2)| < z(\epsilon)$. Draw inspiration from how people minimize the empirical loss in maximizing accuracy. Emphasize that this is only possible due to the way we express our fairness constraint.  (2) The straightforward way is to use a quadratic regularization term $\lambda((L(G1) - L(G2))^2$, ala the L2 normalization. However, this terms becomes very hard to optimize in a model-agnostic way given the quadratic term. We use the linear regularization term $\lambda(L(G1)-L(G2))$ by allowing $\lambda$ to be any real value (positive or negative). This introduces unique challenges in tuning $\lambda$, as we will show later. (3) The regularized objective function can be rearranged into a weighted empirical loss.  
    
    
    \item Tuning $\lambda$. First need to explain the use of a validation set. Then explain the monotonic property, which should be the same for DP or PP. Explain how this unique property can help with hyperparameter tuning. 
    
    \item Explain the tuning algorithm for when weights do not depend on $h$. (1) Determining which direction (positive or negative) we should be searching based on the fairness result when $\lambda =0$; (2) Use exponential search to determine an upper bound or lower bound for $\lambda$; (3) use binary search for finding the optimum $\lambda$. Explain the complexity of the algorithm. Is there any theoretical optimality of our solution that we can say? 
    
    \item Explain the tuning algorithm for when weights depend $h$. Explain the intricacies of the situation. Explain our main insights --- we assume a small enough change in $lambda$ do not affect the example weights. 
\end{itemize}


Having the fairness definition defined in Section~\ref{sec:declarative}, the next step is to transform those formulations into an optimization problem so that we can solve it.
In this section, we introduce how we translate fairness metrics into regularization terms, and eventually makes the whole problem a weighted version of original problem. Here, we assume we only have two groups($g_1$ and $g_2$) and one fairness metric. The extension to multiple groups and multiple fairness metrics is discussed in sec~\ref{sec:mutiple}.



\subsection{Translating to Weighted Version} \label{sec:tech:weigh_translation}
The original optimization problem is defined by:
\begin{equation} \label{equ:original}
        \min_{\theta} \frac{1}{N} \sum_{i=1}^{N} L(x_i,y_i,\theta)  \\
\end{equation}

Where $\theta$ is the model of the classifier \texttt{h}. 

Note that in section~\ref{sec:mlmodels}, we have introduced that in machine learning algorithms, loss functions $L(x_i,y_i,\theta)$ is used as a proxy for accuracy $\mathbbm{1}(h_{\theta}(x_i)=y_i)$. Similarly, if fairness metric defined in section~\ref{sec:declarative_metrics} can be represented by a linear combination of accuracy, we can also use a linear combination of loss to approximate fairness metrics. Also, just like some machine learning models use norms of the model as regularization term, we use fairness metrics as a regularization term to guarantee fairness.
\begin{definition} (Optimization formulation for fairness)\\
\begin{equation}
\label{equation:fairness_opt}
\begin{split}
    \min_{\theta} \frac{1}{N} &\sum_{i=1}^{N} L(x_i,y_i,\theta) + \\
    & \quad \lambda (\sum_{i \in g_1} c_iL(x_i,y_i,\theta)- \sum_{i \in g_2} c_iL(x_i,y_i,\theta))
\end{split}
\end{equation}

\end{definition}
What Equation~\ref{equation:fairness_opt} does is that it takes the difference of fairness metric \texttt{f} of two groups ($g_1$ and $g_2$), use loss function as an proxy to replace the indicator function, and add it to the original optimization problem as a regularization term.

Here, we assume that the the average loss of $g_1$ is greater than $g_2$ and we want to decrease the gap to ensure fairness. Notice that unlike most regularization terms, our regularization term doesn't have absolute value or square and the value of our regularization could be negative. This could potentially make this total loss become negative and if that happens, the best solution would be making the loss negative infinity which doesn't make sense. Also, it could make algorithm tend to give very low loss to $g_1$ and high loss to $g_2$, leading to reverse discrimination. However, we argue that these two problems could be dealt with. First, we limit the value of $\lambda$ to make sure the total loss is still non-negative. Second, we can tune the $\lambda$ in the validation set to make sure that we don't overly enforce fairness to have reverse discrimination, just like tuning other hyper-parameters.

The reason for using this formulation is that we can combine the two accuracy term and the fairness regularization term to make this a weighted version of original optimization problem:
\begin{definition} (Weighted optimization problem)
\begin{equation}
\label{equation:weighted_opt}
\begin{split}
    &\min_{\theta} \frac{1}{N} \sum_{i=1}^{N} L(x_i,y_i,\theta) + \\
    & \quad \lambda (\sum_{i \in g_1} c_iL(x_i,y_i,\theta)- \sum_{i \in g_2} c_iL(x_i,y_i,\theta)) \\
    & =\min_{\theta} (\sum_{i \in g_1} (\frac{1}{N}+\lambda c_i)L(x_i,y_i,\theta)+\sum_{i \in g_2} (\frac{1}{N}-\lambda c_i)L(x_i,y_i,\theta)))\\
    & = \min_{\theta} \frac{1}{N}\sum_{i=1}^{N} w_iL(x_i,y_i,\theta)
\end{split}
\end{equation}
\end{definition}
The Equation~\ref{equation:weighted_opt} gives us a weighted version of the original optimization problem that also considers fairness. If $i \in g_1$, $w_i=1 + \lambda c_i N$, if $i \in g_2$, $w_i=1 - \lambda c_i N$. The $w_i$ for each fairness metric can be computed directly form their corresponding coefficients $c_i$, and we list the weights for the most popular group fairness metrics in Table~\ref{table:weights}. 

We want to make sure that each weight $w_i \geq 0$, which means that $\lambda$ has an upper bound $\lambda \leq \frac{1}{\max|c_i|N}$.
\begin{table*}
\caption{Weights for different popular group fairness metrics. MR: misclassification rate, EO: Equalized Odd, PP: predictive parity, and DP: demographic parity. $pos$ means it is for positive class and $neg$ means it is for negative class. The weights $w_i$ are split into four groups based on their labels $y_i$ and their group $g$.}
\label{table:weights}
\begin{tabular}{|l|l|l|l|l|}
\hline
 & $w_i \vert y_i = 0, g_1 $& $w_i \vert y_i = 1,g_1 $ & $w_i \vert y_i = 0, g_2 $& $w_i \vert y_i = 1,g_2 $ \\ \hline
MR & $1+\frac{\lambda N}{\vert g_1 \vert}$ &  $1+\frac{\lambda N}{\vert g_1 \vert}$ & $1-\frac{\lambda N}{\vert g_2 \vert}$ & $1-\frac{\lambda N}{\vert g_2 \vert}$\\ \hline
$\text{EO}_{pos}$ & 0  & $1+\frac{\lambda N}{\vert \{i : i \in g_1, y_i = 1\} \vert}$ & 0 & $1-\frac{\lambda N}{\vert \{i : i \in g_2, y_i = 1\} \vert}$\\ \hline
$\text{EO}_{neg}$ & $1 + \frac{\lambda N}{\vert \{i : i \in g_1, y_i = 0\} \vert}$  & 0 & $1 - \frac{\lambda N}{\vert \{i : i \in g_2, y_i = 0\} \vert}$ & 0 \\ \hline
$\text{PP}_{pos}$ & 0  & $1 + \frac{\lambda N}{\vert \{i : i \in g_1, h(x_i) = 1\} \vert}$ & 0 & $1 - \frac{\lambda N}{\vert \{i : i \in g_2, h(x_i) = 1\} \vert}$ \\ \hline
$\text{PP}_{neg}$ & $1 + \frac{\lambda N}{\vert \{i : i \in g_1, h(x_i) = 0\} \vert}$  & 0 & $1 - \frac{\lambda N}{\vert \{i : i \in g_2, h(x_i) = 0\} \vert}$ & 0 \\ \hline
DP & $ 1 - \frac{\lambda N}{\vert g_1 \vert}$ & $ 1+ \frac{\lambda N}{\vert g_1 \vert}$ & $1 + \frac{\lambda N}{\vert g_2 \vert}$  & $1 - \frac{\lambda N}{\vert g_2 \vert}$\\ \hline
\end{tabular}
\end{table*}

\subsection{Tuning the \textbf{$\lambda$}}\label{sec:tech:tuning}
Now we have this weighted version of the optimization problem. For each given $\lambda$, we can calculate the weights $w_i$ for each data point and train a model with these new weights. Just like in traditional machine learning we need to tune the weight of regularization term, we need to tune $\lambda$ in our settings on validation set to find the best trade-off between accuracy and fairness that satisfies the constraint. Also, we want to tune the $\lambda$ to make sure that their is no reverse discrimination because our formulation doesn't guarantee that. In this section, we discuss how we tune the $\lambda$ using the validation set.

\subsubsection{Fairness metric whose coefficients don't rely on the prediction $h(x_i)$}

If the fairness metric doesn't involve $h(x_i)$, e.g., Equalized Odds and Demographic Parity, we can directly compute both $\vert G \vert$ and $\vert \{i: i\in g, y_i=1\} \vert$, which means that given a $\lambda$, we can directly compute $w_i$ and train a classifier with the new weights. After training, we can calculate new accuracy and new fairness metric on new weights.

We find that as we increase $\lambda$, the accuracy decreases and the fairness $f(h,g_1) - f(h,g_2)$ decreases.
\begin{proof} 
    Assume we have 
    \begin{equation}
\label{equation:proof}
\begin{split}
    \theta_1 = \argmin_{\theta} \frac{1}{N} &\sum_{i=1}^{N} L(x_i,y_i,\theta) + \\
    & \quad \lambda_1 (\sum_{i \in g_1} c_iL(x_i,y_i,\theta)- \sum_{i \in g_2} c_iL(x_i,y_i,\theta)) \\
    \theta_2 = \argmin_{\theta} \frac{1}{N} &\sum_{i=1}^{N} L(x_i,y_i,\theta) + \\
    & \quad \lambda_2 (\sum_{i \in g_1} c_iL(x_i,y_i,\theta)- \sum_{i \in g_2} c_iL(x_i,y_i,\theta))
\end{split}
\end{equation}
Where $\lambda_2 > \lambda_1 \geq 0$, for simplicity, we use $L_1(\theta)$ to represent \\$\frac{1}{N} \sum_{i=1}^{N} L(x_i,y_i,\theta)$, and $L_2(\theta)$ to represent $(\sum_{i \in g_1} c_iL(x_i,y_i,\theta)- \sum_{i \in g_2} c_iL(x_i,y_i,\theta))$.
Then,
\begin{equation}
    \label{equ:lambda1}
    L_1(\theta_1) + \lambda_1 L_2(\theta_1) \leq  L_1(\theta_2) + \lambda_1 L_2(\theta_2)
\end{equation}
\begin{equation}
    \label{equ:lambda2}
    L_1(\theta_2) + \lambda_2 L_2(\theta_2) \leq  L_1(\theta_1) + \lambda_2 L_2(\theta_1)
\end{equation}
Adding Equation~\ref{equ:lambda1} and~\ref{equ:lambda2}, we have
\begin{equation}
    \lambda_1 L_2(\theta_1) + \lambda_2 L_2(\theta_2) \leq  \lambda_1 L_2(\theta_2) + \lambda_2 L_2(\theta_1)
\end{equation}
Shuffling the terms and we get
\begin{equation}
    (\lambda_2 - \lambda_1)(L_2(\theta_1) -L_2(\theta_2) ) \geq 0
\end{equation}
Given that $\lambda_2 \geq \lambda_1$, we have $L_2(\theta_1) -L_2(\theta_2) \geq 0$, meaning that the loss for the fairness cannot increase after we increase $\lambda$. We take this back to Equation~\ref{equ:lambda1}, and gets that $L_1(\theta_1) \leq  L_1(\theta_2)$, meaning that the loss for accuracy cannot decrease after we increase $\lambda$.
\end{proof}

 \todo{add a proof for monotonicity of tuning lambda and/or a micro-experiment showing the monotonicity. Proof is done, need to write it here} Based on this observation, we can do a binary search on $\lambda$ between $[0, \frac{1}{\max|c_i|N}]$ to find the best $\lambda$ that maximizes accuracy while satisfying the fairness constraint and not introducing reverse discrimination.
 
 % --- New theorems added here




\subsubsection{Fairness metric whose coefficients rely on the prediction $h(x_i)$}

However, if the fairness metric is based on the prediction $h(x_i)$ like predictive parity, we need to compute $\vert \{i: i\in g, h(x_i)=1\} \vert$ to get weights $w_i$. 
The $h(x_i)$ would change after we update the weights and retrain the model with new weights, so our estimation using old $h(x_i)$ may not be accurate. To deal with this problem, we come up with an iterative algorithm that keeps retraining until all predictions of the model doesn't change, this ensures that our estimation of $\vert \{i: i\in g, h(x_i)=1\} \vert$ is accurate. The detail is shown in algorithm~\ref{alg:itertune}.

\begin{algorithm}
\label{alg:itertune}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{A classifier h, a dataset D }
 \Output{weights $w_i$}
 $h_{new}$ = NULL;
 
 \While{$\exists i \in D, h(x_i) \neq h_{new}(x_i)$}{
  $h$ = $h_{new}$;
  
  calculate $\vert \{i: i\in g, h(x_i)=1\} \vert$ and use it to get new weights $w_i$;
  
  Train $h_{new}$ using new weights $w_i$;
  
 }
 \caption{Tuning $\lambda$ when the fairness metric relys on predictions}
\end{algorithm}

With this algorithm, we can get the correct weights $w_i$ for each $\lambda$, and the monotonicity also holds in this case. Similar to the previous case, we do a binary search on $\lambda$ to find the best accuracy that satisfies the fairness constraints.
